The role of pressure-induced stacking faults on the magnetic properties of gadolinium

Experimental data show that under pressure, Gd goes through a series of structural transitions hcp to Sm-type (close-packed rhombohedral) to dhcp that is accompanied by a gradual decrease of the Curie temperature and magnetization till the collapse of a finite magnetization close to the dhcp structure. We explore theoretically the pressure-induced changes of the magnetic properties, by describing these structural transitions as the formation of fcc stackings faults. Using this approach, we are able to describe correctly the variation of the Curie temperature with pressure, in contrast to a static structural model using the hcp structure.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
